Opti-CAM: Optimizing saliency maps for interpretability

Methods based on class activation maps (CAM) provide a simple mechanism to interpret predictions of convolutional neural networks by using linear combinations of feature maps as saliency maps. By contrast, masking-based methods optimize a saliency map directly in the image space or learn it by training another network on additional data. In this work we introduce Opti-CAM, combining ideas from CAM-based and masking-based approaches. Our saliency map is a linear combination of feature maps, where weights are optimized per image such that the logit of the masked image for a given class is maximized. We also fix a fundamental flaw in two of the most common evaluation metrics of attribution methods. On several datasets, Opti-CAM largely outperforms other CAM-based approaches according to the most relevant classification metrics. We provide empirical evidence supporting that localization and classifier interpretability are not necessarily aligned.

==> tex/plots-ext.tex <==
%------------------------------------------------------------------------------
% hack for CVPR/ICCV style
% \makeatletter
% \@namedef{ver@everyshi.sty}{}
% \makeatother

%------------------------------------------------------------------------------
% main packages
\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{tikzextern}
\usepackage{pgffor}

%------------------------------------------------------------------------------
% externalization
\newcommand{\extfig}[2]{\tikzsetnextfilename{fig/extern/#1}{#2}}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> tex/plots-none.tex <==
\newcommand{\extfig}[2]{!!!}
\newcommand{\noextfig}[1]{!!!}
\newcommand{\extdata}[1]{}


==> tex/show_image_deit.tex <==
\begin{figure*}[t]
\newcommand{\sizeP}{.12}
\newcommand{\sizeS}{.12}
\newcommand{\hh}{.175\textwidth}
\newcommand{\ww}{.200\textwidth}
\tiny
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{cccccccc}
	Input image  &  Grad-CAM  & G-CAM++ & Score-CAM & XG-CAM & Raw Att. & Rollout & Opti-CAM (ours) \\
        \includegraphics[trim={12mm 14mm 12mm 14mm},clip, width=\sizeP\textwidth]{fig/visual/ILSVRC2012_val_00000089.JPEG}&
	\fig[\sizeS]{visual/DeitBase_GradCAM_ILSVRC2012_val_00000089.png} &
	\fig[\sizeS]{visual/DeitBase_GradCAMPlusPlus_ILSVRC2012_val_00000089.png} &
	\fig[\sizeS]{visual/DeitBase_ScoreCAM_ILSVRC2012_val_00000089.png} &
	\fig[\sizeS]{visual/DeitBase_XGradCAM_ILSVRC2012_val_00000089.png} & 
        \fig[\sizeS]{visual/DeitBase_RawAttention_ILSVRC2012_val_00000089.png} &
        \fig[\sizeS]{visual/DeitBase_RolloutMean_ILSVRC2012_val_00000089.png} &
	\fig[\sizeS]{visual/DeitBase_OptiCAM_ILSVRC2012_val_00000089.png}  \\
	Cellphone &&&&&& \\
	\fig[\sizeS]{visual/ILSVRC2012_val_00000748.png}&
	\fig[\sizeS]{visual/DeitBase_GradCAM_ILSVRC2012_val_00000748.png} &
	\fig[\sizeS]{visual/DeitBase_GradCAMPlusPlus_ILSVRC2012_val_00000748.png} &
	\fig[\sizeS]{visual/DeitBase_ScoreCAM_ILSVRC2012_val_00000748.png} &
	\fig[\sizeS]{visual/DeitBase_XGradCAM_ILSVRC2012_val_00000748.png} & 
        \fig[\sizeS]{visual/DeitBase_RawAttention_ILSVRC2012_val_00000748.png} &
        \fig[\sizeS]{visual/DeitBase_RolloutMean_ILSVRC2012_val_00000748.png} &
	\fig[\sizeS]{visual/DeitBase_OptiCAM_ILSVRC2012_val_00000748.png}  \\
	Miniature Schnauzer &&&&&& \\
	\includegraphics[trim={2mm 3mm 6mm 1mm},clip, width=\sizeP\textwidth]{fig/visual/ILSVRC2012_val_00000769.JPEG}&
	\fig[\sizeS]{visual/DeitBase_GradCAM_ILSVRC2012_val_00000769.png} &
	\fig[\sizeS]{visual/DeitBase_GradCAMPlusPlus_ILSVRC2012_val_00000769.png} &
	\fig[\sizeS]{visual/DeitBase_ScoreCAM_ILSVRC2012_val_00000769.png} &
	\fig[\sizeS]{visual/DeitBase_XGradCAM_ILSVRC2012_val_00000769.png} & 
        \fig[\sizeS]{visual/DeitBase_RawAttention_ILSVRC2012_val_00000769.png} &
        \fig[\sizeS]{visual/DeitBase_RolloutMean_ILSVRC2012_val_00000769.png} &
	\fig[\sizeS]{visual/DeitBase_OptiCAM_ILSVRC2012_val_00000769.png}  \\
	Face Powder &&&&&& \\
	\includegraphics[trim={2mm 6mm 2mm 6mm},clip, width=\sizeP\textwidth]{fig/visual/ILSVRC2012_val_00000782.JPEG}&
	\fig[\sizeS]{visual/DeitBase_GradCAM_ILSVRC2012_val_00000782.png} &
	\fig[\sizeS]{visual/DeitBase_GradCAMPlusPlus_ILSVRC2012_val_00000782.png} &
	\fig[\sizeS]{visual/DeitBase_ScoreCAM_ILSVRC2012_val_00000782.png} &
	\fig[\sizeS]{visual/DeitBase_XGradCAM_ILSVRC2012_val_00000782.png} & 
        \fig[\sizeS]{visual/DeitBase_RawAttention_ILSVRC2012_val_00000782.png} &
        \fig[\sizeS]{visual/DeitBase_RolloutMean_ILSVRC2012_val_00000782.png} &
	\fig[\sizeS]{visual/DeitBase_OptiCAM_ILSVRC2012_val_00000782.png}  \\
	Chocolate Sauce &&&&&& \\
	\fig[\sizeS]{visual/ILSVRC2012_val_00001113.png}&
	\fig[\sizeS]{visual/DeitBase_GradCAM_ILSVRC2012_val_00001113.png} &
	\fig[\sizeS]{visual/DeitBase_GradCAMPlusPlus_ILSVRC2012_val_00001113.png} &
	\fig[\sizeS]{visual/DeitBase_ScoreCAM_ILSVRC2012_val_00001113.png} &
	\fig[\sizeS]{visual/DeitBase_XGradCAM_ILSVRC2012_val_00001113.png} & 
        \fig[\sizeS]{visual/DeitBase_RawAttention_ILSVRC2012_val_00001113.png} &
        \fig[\sizeS]{visual/DeitBase_RolloutMean_ILSVRC2012_val_00001113.png} &
	\fig[\sizeS]{visual/DeitBase_OptiCAM_ILSVRC2012_val_00001113.png}  \\
	Komondor &&&&&& \\
 \includegraphics[trim={14mm 16mm 14mm 12mm},clip, width=\sizeP\textwidth]{fig/visual/ILSVRC2012_val_00001345.JPEG}&
	\fig[\sizeS]{visual/DeitBase_GradCAM_ILSVRC2012_val_00001345.png} &
	\fig[\sizeS]{visual/DeitBase_GradCAMPlusPlus_ILSVRC2012_val_00001345.png} &
	\fig[\sizeS]{visual/DeitBase_ScoreCAM_ILSVRC2012_val_00001345.png} &
	\fig[\sizeS]{visual/DeitBase_XGradCAM_ILSVRC2012_val_00001345.png} & 
        \fig[\sizeS]{visual/DeitBase_RawAttention_ILSVRC2012_val_00001345.png} &
        \fig[\sizeS]{visual/DeitBase_RolloutMean_ILSVRC2012_val_00001345.png} &
	\fig[\sizeS]{visual/DeitBase_OptiCAM_ILSVRC2012_val_00001345.png}  \\
	Quill &&&&&& \\
 \includegraphics[trim={5mm 14mm 5mm 14mm},clip, width=\sizeP\textwidth]{fig/visual/ILSVRC2012_val_00001529.JPEG}&
	\fig[\sizeS]{visual/DeitBase_GradCAM_ILSVRC2012_val_00001529.png} &
	\fig[\sizeS]{visual/DeitBase_GradCAMPlusPlus_ILSVRC2012_val_00001529.png} &
	\fig[\sizeS]{visual/DeitBase_ScoreCAM_ILSVRC2012_val_00001529.png} &
	\fig[\sizeS]{visual/DeitBase_XGradCAM_ILSVRC2012_val_00001529.png} & 
        \fig[\sizeS]{visual/DeitBase_RawAttention_ILSVRC2012_val_00001529.png} &
        \fig[\sizeS]{visual/DeitBase_RolloutMean_ILSVRC2012_val_00001529.png} &
	\fig[\sizeS]{visual/DeitBase_OptiCAM_ILSVRC2012_val_00001529.png}  \\
	Longicorn &&&&&& \\
 \includegraphics[trim={8mm 1mm 8mm 1mm},clip, width=\sizeP\textwidth]{fig/visual/ILSVRC2012_val_00001635.JPEG}&
	\fig[\sizeS]{visual/DeitBase_GradCAM_ILSVRC2012_val_00001635.png} &
	\fig[\sizeS]{visual/DeitBase_GradCAMPlusPlus_ILSVRC2012_val_00001635.png} &
	\fig[\sizeS]{visual/DeitBase_ScoreCAM_ILSVRC2012_val_00001635.png} &
	\fig[\sizeS]{visual/DeitBase_XGradCAM_ILSVRC2012_val_00001635.png} & 
        \fig[\sizeS]{visual/DeitBase_RawAttention_ILSVRC2012_val_00001635.png} &
        \fig[\sizeS]{visual/DeitBase_RolloutMean_ILSVRC2012_val_00001635.png} &
	\fig[\sizeS]{visual/DeitBase_OptiCAM_ILSVRC2012_val_00001635.png}  \\
	Slide Rule &&&&&& \\
\end{tabular}
\vspace{5pt}
\caption{Saliency maps obtained from ImageNet example images using different methods on DeiT.}
\label{fig:imagenet-vis-more-DeiT}
\end{figure*}


==> tex/show_image_deitTiny.tex <==
\begin{figure*}[t]
\newcommand{\sizeP}{.12}
\newcommand{\sizeS}{.12}
\newcommand{\hh}{.175\textwidth}
\newcommand{\ww}{.200\textwidth}
\tiny
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{cccccccc}
	Input image  &  Grad-CAM  & G-CAM++ & Score-CAM & XG-CAM & Raw Att. & Rollout & Opti-CAM (ours) \\
        \includegraphics[trim={12mm 14mm 12mm 14mm},clip, width=\sizeP\textwidth]{fig/visual/ILSVRC2012_val_00000089.JPEG}&
	\fig[\sizeS]{visual/DeitTiny_GradCAM_ILSVRC2012_val_00000089.png} &
	\fig[\sizeS]{visual/DeitTiny_GradCAMPlusPlus_ILSVRC2012_val_00000089.png} &
	\fig[\sizeS]{visual/DeitTiny_ScoreCAM_ILSVRC2012_val_00000089.png} &
	\fig[\sizeS]{visual/DeitTiny_XGradCAM_ILSVRC2012_val_00000089.png} & 
        \fig[\sizeS]{visual/DeitTiny_RawAttention_ILSVRC2012_val_00000089.png} &
        \fig[\sizeS]{visual/DeitTiny_RolloutMean_ILSVRC2012_val_00000089.png} &
	\fig[\sizeS]{visual/DeitTiny_OptiCAM_ILSVRC2012_val_00000089.png}  \\
	Cellphone &&&&&& \\
	\fig[\sizeS]{visual/ILSVRC2012_val_00000748.png}&
	\fig[\sizeS]{visual/DeitTiny_GradCAM_ILSVRC2012_val_00000748.png} &
	\fig[\sizeS]{visual/DeitTiny_GradCAMPlusPlus_ILSVRC2012_val_00000748.png} &
	\fig[\sizeS]{visual/DeitTiny_ScoreCAM_ILSVRC2012_val_00000748.png} &
	\fig[\sizeS]{visual/DeitTiny_XGradCAM_ILSVRC2012_val_00000748.png} & 
        \fig[\sizeS]{visual/DeitTiny_RawAttention_ILSVRC2012_val_00000748.png} &
        \fig[\sizeS]{visual/DeitTiny_RolloutMean_ILSVRC2012_val_00000748.png} &
	\fig[\sizeS]{visual/DeitTiny_OptiCAM_ILSVRC2012_val_00000748.png}  \\
	Miniature Schnauzer &&&&&& \\
	\includegraphics[trim={2mm 3mm 6mm 1mm},clip, width=\sizeP\textwidth]{fig/visual/ILSVRC2012_val_00000769.JPEG}&
	\fig[\sizeS]{visual/DeitTiny_GradCAM_ILSVRC2012_val_00000769.png} &
	\fig[\sizeS]{visual/DeitTiny_GradCAMPlusPlus_ILSVRC2012_val_00000769.png} &
	\fig[\sizeS]{visual/DeitTiny_ScoreCAM_ILSVRC2012_val_00000769.png} &
	\fig[\sizeS]{visual/DeitTiny_XGradCAM_ILSVRC2012_val_00000769.png} & 
        \fig[\sizeS]{visual/DeitTiny_RawAttention_ILSVRC2012_val_00000769.png} &
        \fig[\sizeS]{visual/DeitTiny_RolloutMean_ILSVRC2012_val_00000769.png} &
	\fig[\sizeS]{visual/DeitTiny_OptiCAM_ILSVRC2012_val_00000769.png}  \\
	Face Powder &&&&&& \\
	\includegraphics[trim={2mm 6mm 2mm 6mm},clip, width=\sizeP\textwidth]{fig/visual/ILSVRC2012_val_00000782.JPEG}&
	\fig[\sizeS]{visual/DeitTiny_GradCAM_ILSVRC2012_val_00000782.png} &
	\fig[\sizeS]{visual/DeitTiny_GradCAMPlusPlus_ILSVRC2012_val_00000782.png} &
	\fig[\sizeS]{visual/DeitTiny_ScoreCAM_ILSVRC2012_val_00000782.png} &
	\fig[\sizeS]{visual/DeitTiny_XGradCAM_ILSVRC2012_val_00000782.png} & 
        \fig[\sizeS]{visual/DeitTiny_RawAttention_ILSVRC2012_val_00000782.png} &
        \fig[\sizeS]{visual/DeitTiny_RolloutMean_ILSVRC2012_val_00000782.png} &
	\fig[\sizeS]{visual/DeitTiny_OptiCAM_ILSVRC2012_val_00000782.png}  \\
	Chocolate Sauce &&&&&& \\
	\fig[\sizeS]{visual/ILSVRC2012_val_00001113.png}&
	\fig[\sizeS]{visual/DeitTiny_GradCAM_ILSVRC2012_val_00001113.png} &
	\fig[\sizeS]{visual/DeitTiny_GradCAMPlusPlus_ILSVRC2012_val_00001113.png} &
	\fig[\sizeS]{visual/DeitTiny_ScoreCAM_ILSVRC2012_val_00001113.png} &
	\fig[\sizeS]{visual/DeitTiny_XGradCAM_ILSVRC2012_val_00001113.png} & 
        \fig[\sizeS]{visual/DeitTiny_RawAttention_ILSVRC2012_val_00001113.png} &
        \fig[\sizeS]{visual/DeitTiny_RolloutMean_ILSVRC2012_val_00001113.png} &
	\fig[\sizeS]{visual/DeitTiny_OptiCAM_ILSVRC2012_val_00001113.png}  \\
	Komondor &&&&&& \\
 \includegraphics[trim={14mm 16mm 14mm 12mm},clip, width=\sizeP\textwidth]{fig/visual/ILSVRC2012_val_00001345.JPEG}&
	\fig[\sizeS]{visual/DeitTiny_GradCAM_ILSVRC2012_val_00001345.png} &
	\fig[\sizeS]{visual/DeitTiny_GradCAMPlusPlus_ILSVRC2012_val_00001345.png} &
	\fig[\sizeS]{visual/DeitTiny_ScoreCAM_ILSVRC2012_val_00001345.png} &
	\fig[\sizeS]{visual/DeitTiny_XGradCAM_ILSVRC2012_val_00001345.png} & 
        \fig[\sizeS]{visual/DeitTiny_RawAttention_ILSVRC2012_val_00001345.png} &
        \fig[\sizeS]{visual/DeitTiny_RolloutMean_ILSVRC2012_val_00001345.png} &
	\fig[\sizeS]{visual/DeitTiny_OptiCAM_ILSVRC2012_val_00001345.png}  \\
	Quill &&&&&& \\
 \includegraphics[trim={5mm 14mm 5mm 14mm},clip, width=\sizeP\textwidth]{fig/visual/ILSVRC2012_val_00001529.JPEG}&
	\fig[\sizeS]{visual/DeitTiny_GradCAM_ILSVRC2012_val_00001529.png} &
	\fig[\sizeS]{visual/DeitTiny_GradCAMPlusPlus_ILSVRC2012_val_00001529.png} &
	\fig[\sizeS]{visual/DeitTiny_ScoreCAM_ILSVRC2012_val_00001529.png} &
	\fig[\sizeS]{visual/DeitTiny_XGradCAM_ILSVRC2012_val_00001529.png} & 
        \fig[\sizeS]{visual/DeitTiny_RawAttention_ILSVRC2012_val_00001529.png} &
        \fig[\sizeS]{visual/DeitTiny_RolloutMean_ILSVRC2012_val_00001529.png} &
	\fig[\sizeS]{visual/DeitTiny_OptiCAM_ILSVRC2012_val_00001529.png}  \\
	Longicorn &&&&&& \\
 \includegraphics[trim={8mm 1mm 8mm 1mm},clip, width=\sizeP\textwidth]{fig/visual/ILSVRC2012_val_00001635.JPEG}&
	\fig[\sizeS]{visual/DeitTiny_GradCAM_ILSVRC2012_val_00001635.png} &
	\fig[\sizeS]{visual/DeitTiny_GradCAMPlusPlus_ILSVRC2012_val_00001635.png} &
	\fig[\sizeS]{visual/DeitTiny_ScoreCAM_ILSVRC2012_val_00001635.png} &
	\fig[\sizeS]{visual/DeitTiny_XGradCAM_ILSVRC2012_val_00001635.png} & 
        \fig[\sizeS]{visual/DeitTiny_RawAttention_ILSVRC2012_val_00001635.png} &
        \fig[\sizeS]{visual/DeitTiny_RolloutMean_ILSVRC2012_val_00001635.png} &
	\fig[\sizeS]{visual/DeitTiny_OptiCAM_ILSVRC2012_val_00001635.png}  \\
	Slide Rule &&&&&& \\
\end{tabular}
\vspace{5pt}
\caption{Saliency maps obtained from ImageNet example images using different methods on DeitTiny.}
\label{fig:imagenet-vis-more-DeitTiny}
\end{figure*}

